Active Model Estimation in Markov Decision Processes

We study the problem of efficient exploration in order to learn an accurate model of an environment, modeled as a Markov decision process (MDP). Efficient exploration in this problem requires the agent to identify the regions in which estimating the model is more difficult and then exploit this knowledge to collect more samples there. In this paper, we formalize this problem, introduce the first algorithm to learn an $\epsilon$-accurate estimate of the dynamics, and provide its sample complexity analysis. While this algorithm enjoys strong guarantees in the large-sample regime, it tends to have a poor performance in early stages of exploration. To address this issue, we propose an algorithm that is based on maximum weighted entropy, a heuristic that stems from common sense and our theoretical analysis. The main idea here is to cover the entire state-action space with the weight proportional to the noise in the transitions. Using a number of simple domains with heterogeneous noise in their transitions, we show that our heuristic-based algorithm outperforms both our original algorithm and the maximum entropy algorithm in the small sample regime, while achieving similar asymptotic performance as that of the original algorithm.

==> NewMacros.tex <==
%-------------------------------------------------------------------------------
% BASIC COMMANDS

%parantheses
\newcommand{\lp}{\left (}
\newcommand{\rp}{\right )} 
%brackets
\newcommand{\lb}{\left [}
\newcommand{\rb}{\right]} 
% 
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}} 
\newcommand{\reals}{\mathbb{R}} 


\newcommand{\tbf}[1]{\textbf{#1}}

% COLOURED TEXT
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%-------------------------------------------------------------------------------
% ARGMIN AND ARGMAX
%-------------------------------------------------------------------------------
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%-------------------------------------------------------------------------------

% OBJECTIVE FUNCTIONS
\newcommand{\objunif}[1]{\widetilde{\mc{W}}\lp #1 \rp}

%-------------------------------------------------------------------------------
% Best Stationary distribution
\newcommand{\OptDist}{\lambda^*} 
% all feasible lambda values for P in \mathcal{C}_t
\newcommand{\FeasDists}{\Lambda_{\mc{C}_k}}
% 

%-------------------------------------------------------------------------------
% Adaptive Sampling Algorithm 
\newcommand{\algo}[1][]{\mc{A}_{#1}}

%  Regret 
\newcommand{\reg}[1]{\mathcal{R}_{#1}} 

%-------------------------------------------------------------------------------
% BIG OH 
\newcommand{\Oh}[1]{\mathcal{O}\lp #1 \rp}
\newcommand{\tOh}[1]{\tilde{\mathcal{O}} \lp #1 \rp }
%-------------------------------------------------------------------------------


%-------------------------------------------------------------------------------
% REFERENCING 
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}} 
\newcommand{\lemmaref}[1]{Lemma~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}} 
\newcommand{\assumpref}[1]{Assumption~\ref{#1}}
%-------------------------------------------------------------------------------

==> UniformLoss.tex <==
% Preliminaries 
%--------------------------------------------------------------------------------
In light of Eq.~\eqref{obj_2}, we first introduce the uniform estimation objective function $\objunif{\lambda}$ as follows:
\begin{align*}
    \objunif{\lambda} \coloneqq \max_{(s,a) \in \mc{S} \times \mc{A}}\; \frac{ c_{s,a}}{  \lambda(s,a)^\alpha }, 
\end{align*}
where $\alpha >0$, and $c_{s,a}$ is a function of the distribution $p(\cdot \vert s,a)$. Note that $\objunif{\lambda}$ is a convex function of $\lambda$ as it is the maximum of $S\times A$ convex functions. 

We introduce some additional notations and definitions: 
\begin{itemize} 
\item We use $\Lambda_P$ to denote the set of feasible state action stationary distributions, corresponding to any tensor of transition probability vectors $P = \{p(\cdot|s,a), \text{for } (s,a) \in \mc{S}\times \mc{A}\}$. 
\item We use $\mc{C}_k$ to denote the confidence set containing the true model at round $k$. 
\item We use $\FeasDists$ to denote set of all possible state-action stationary distributions corresponding to all models lying in $\mc{C}_k$. 
\item We use $\OptDist$, to denote $\argmin_{\lambda \in \Lambda_P}\; \objunif{\lambda}$, where $P$ denotes the true underlying model. 
\item Suppose any adaptive allocation policy results in an empirical state-action distribution $\hat{\lambda}_k$ at the end of $k$ rounds/episodes, then we define the (pseudo-)regret as $\reg{k} \coloneqq \objunif{\hat{\lambda}_k} - \objunif{\OptDist}$. 
\end{itemize}

%--------------------------------------------------------------------------------
% ALGORITHM
%--------------------------------------------------------------------------------
\subsection{Algorithm}
\label{subsec:UniformAlgorithm}

We now describe the algorithm for estimating the model of an MDP uniformly well, motivated by the analogous algorithm from the bandit setting~\citep{shekhar2019adaptive}. The general idea is to construct an optimistic estimate of the objective function by replacing the true parameter $c_{s,a}$ by its current UCB $\hat{u}_{k,s,a}$ and then select a policy which visits the $(s,a)$ for which this value is maximum. In the bandit setting, we can select specific arms to play, according the rule $\argmax_{(s,a)} \hat{u}_{k,s,a}/\hat{\lambda}_k(s,a)^\alpha = \argmax_{\lambda \in \Delta_{S\times A}} \sum_{s,a} \lambda(s,a) \frac{\hat{u}_{k,s,a}}{\hat{\lambda}_k(s,a)^\alpha}$. This step is replaced by Line~4-5, which is the main algorithmic modification. 

In the algorithm, $\tau_1$ is the random time that is required for some chosen policy $\pi_0$ to visit each $(s,a)$ pair at least once. 

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\SetKwFunction{Expand}{Expand}
\newcommand\mycommfont[1]{\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}


\KwIn{$n$, $\lp \tau_k\rp_{k \geq 1}$}
 \tbf{Initialize:}~ $k=1$, $\tau_1$, $\hat{\lambda}_1$,  $\mc{C}_k$, \;
 % BEGIN FOR LOOP
\For{$k=1,2,\ldots$}
{ 
Construct UCB $\hat{u}_{k,s,a}$ of $c_{s,a}$ for all $(s,a) \in \mc{S}\times \mc{A}$\\
% \tcp{Optimistic subgradient direction}
\tcp{Choose a state-action pair optimistically}
$(s_k, a_k) = \argmax_{(s,a) \in \mc{S}\times \mc{A}}\, \frac{\hat{u}_{k,s,a}}{\hat{\lambda}_k(s,a)^\alpha}$ \\
% \tcp{Projection Step}
\tcp{Solve the extended average cost MDP}
Choose $\lambda_k \in \argmax_{\lambda \in \FeasDists} \, \lambda(s_k,a_k)$ \\
% \frac{\hat{u}_{k,s,a}}{\hat{\lambda}_k(s,a)^{\alpha+1}}$ \\
Define policy $\pi_k$ corresponding to $\lambda_k$ \\
Play $\pi_k$ for $\tau_k$ steps \\
Update $\hat{u}_{k,s,a}$ and $\mc{C}_k$. 

} 
\caption{}
\label{algo:uniform}
\end{algorithm}





%--------------------------------------------------------------------------------
% ANALYSIS
%--------------------------------------------------------------------------------
\subsection{Analysis}
\label{subsec:AnalysisUniform}

For now, we work under Assumption~2 of \citep{tarbouriech2019active}, which assumes that the true model is such that any stationary policy induces an ergodic Markov chain. 

The following components will have to be controlled to obtain the regret bound:
\begin{itemize} 
\item Confidence interval length for estimation of $c_{s,a}$ for $(s,a) \in S\times A$. \blue{(In our case, this will follow from confidence intervals  of the  variances)} 
\item Deviation between $\lambda_k$~(Line~4-5 of \algoref{algo:uniform}) and $\tilde{\lambda}_k \coloneqq \argmax_{\lambda \in \FeasDists} \sum_{s,a} \lambda(s,a) \frac{c_{s,a}}{\hat{\lambda}_k(s,a)^\alpha}$. 
\blue{(That is, $\tilde{\lambda}_k$ is the distribution assuming the knowledge of true $c_{s,a}$ in Line~4-5.)} 

\item Deviation between $\tilde{\lambda}_k$ and $\bar{\lambda}_k \coloneqq \argmax_{\lambda \in \Lambda} \sum_{s,a} \lambda(s,a) \frac{c_{s,a}}{\hat{\lambda}_k(s,a)^\alpha}$. 
\blue{($\bar{\lambda}_k$ is the distribution assuming knowledge of the true model.)}

\item Deviation between $\lambda_k$ and the actual empirical distribution induced in the episode $k$, denoted by $\psi_k$. \blue{(This is controlled by Prop.~1) of \cite{tarbouriech2019active})}
\end{itemize} 



